Can AI Prompt Humans? Multimodal Agents Prompt Players' Game Actions and Show Consequences to Raise Sustainability Awareness

Unsustainable behaviors are challenging to prevent due to their long-term, often unclear consequences. Games offer a promising solution by creating artificial environments where players can immediately experience the outcomes of their actions. To explore this potential, we developed EcoEcho, a GenAI-powered game leveraging multimodal agents to raise sustainability awareness. These agents engage players in natural conversations, prompting them to take in-game actions that lead to visible environmental impacts. We evaluated EcoEcho using a mixed-methods approach with 23 participants. Results show a significant increase in intended sustainable behaviors post-game, although attitudes towards sustainability only slightly improved. This finding highlights the potential of multimodal agents and action-consequence mechanics to effectively motivate real-world behavioral changes such as raising environmental sustainability awareness.

==> mainacm.tex <==
\newcommand{\remove}[1]{{\color{red} \sout{#1}}}
%\newcommand{\change}[1]{{\color{blue} \uwave{#1}}}
\newcommand{\change}[1]{{\color{blue} #1}}


==> sections/prev-01-Intro.tex <==
% \begin{figure*}[htbp]
%   \centering
%   \includegraphics[height=0.5\textheight, width=0.8\textwidth, keepaspectratio]{figs/GameStart.png}
%   \caption{EcoEcho. A Role Playing AI Game for Promoting the Awareness of Sustainable Behavior.}
%   \label{fig:gamestart}
%   \Description{Caption}
% \end{figure*}

%motivation: future thinking, negative behaviors consequences. can talk about indiv differences and how effect could be diff on their behaviors. or say you can prevent one person but not another.
%1. temporal, 2. indiv diff.
Preventing unsustainable human behaviors has long been a challenge due to humanity's inherent predisposition towards actions driven by short-term individual interests, coupled with the ambiguous nature of the long-term consequences associated with unsustainable practices ~\cite{gual2010bridging,damasio1994descartes}
. \ad{Previous Research has shown nuanced relationships between \textbf{sustainability awareness, attitude, and behavior}. For instance, Arshad et al. 
~\cite{arshad2021environmental} found that awareness and attitudes do not always correlate. However, studies by Gao ~\cite{firmanshah2023relationship} and Safari et al. ~\cite{cogut2019links} have consistently reported a positive correlation between sustainability awareness and sustainable behavior. Individual differences in personality and attitudes influence receptiveness to sustainability goals, ultimately shaping engagement and commitment to sustainable behaviors~\cite{zhou2024eternagram}.} Therefore, merely emphasizing the importance of sustainability fails to engender a visceral understanding among individuals. While humans are most profoundly influenced by experiencing the adverse outcomes or even failures resulting from their own actions, replicating such scenarios in the real world is neither feasible nor sufficiently protective of the environment.

%need to discuss their indiv difference, how engagement affects them differently, and how their attitudes may be leading to different levels of commitment or action.


%games a way to raise awareness by artificial incentivizing posistives and discouraging negatives. evidence for why games are effective. cite games (eternagram). set up the fact that it's hard to design a realistic game (problem 1). how do we we convert game behavior into real behavior? (problem 2)

% [games, conversation with NPC, but rubric-based]

Games are a method to raise awareness by artificially incentivizing positive factors and inhibiting negative ones, offering a quick and intuitive way for people to immediately see the consequences of their actions. \ad{Our game is designed to raise \textbf{sustainability awareness,}} players can experience the impact of their behaviors through role-playing and interaction, which is often difficult to perceive immediately in real life ~\cite{juul2013art}. Meanwhile, traditional game design often relies on preset text options and limited interaction methods, restricting players' behavioral expression and failing to fully reflect their real-life intentions and actions. Although gamified interventions can effectively increase players' environmental awareness and promote more positive behavioral intentions ~\cite{juan2015game,zhou2024eternagram}, there still exists a discrepancy between behaviors in virtual environments and those in real life.

% \textcolor{blue}{(people don't really do in real life what they do in the game)}.

%GenAI allows realistic convo (NLP), real characters, therefore more like real world. (address problem 1)

%people don't really do in real life what they do in the game, so GenAI strategy for converting verbal behavior in game into actual behavior in game to mimick real world situation. (problem 2) rationale for why do the words into action: to encourage people to do what they say in the real world.

% [Multi-modal generative AI addresses the problem in previous games of influencing user behaviors]

% The advent of multimodal capabilities in Generative AI (GenAI) presents new opportunities for simulating the harmful consequences of human behavior ~\cite{park2023generative,link2016intelligent,holmgard2014generative}.
The advent of Generative AI  \cite{feuerriegel2024generative}, particularly the advanced natural language processing capabilities of language models, offers new avenues for simulating the harmful consequences of human  behavior~\cite{park2023generative,link2016intelligent,holmgard2014generative}. We built EcoEcho, a virtual game environment that synthesizes visual, auditory, and narrative modalities to immerse players in the role of a conflicted scientist whose misinterpretation of his father's dying wish leads him to impede clean energy advancement. To drive the plot forward, we harness GenAI’s ability to elicit natural language responses from players and seamlessly translate those verbal inputs into corresponding in-game actions. Through dynamic interactions with various stakeholders, such as journalists, union leaders, and ministers of energy, players engage in unsustainable behaviors within the game world, turning conversational choices into tangible consequences. By experiencing the negative outcomes of these actions, the game aims to increase awareness of sustainability issues both in-game and in real life.


% capabilities enables realistic conversations and lifelike characters, closely mimicking real-world Human-to-Human Interactions. Additionally, GenAI's multimodal capabilities present new opportunities for simulating the harmful consequences of human behavior~\cite{park2023generative,link2016intelligent,holmgard2014generative}. }

% We built a virtual game environment EcoEcho that leverages multimodal GenAI to facilitate dynamic interactions between players and AI-driven avatars. EcoEcho synthesizes visual, auditory, and narrative modalities to immerse players in the role of a conflicted scientist whose misinterpretation of his father's dying wish leads him to impede clean energy advancement. Through dialogues with multiple stakeholders, such as journalists, union leaders, and ministers of energy, the game design engages players in unsustainable behaviors within the virtual world. By demonstrating the negative consequences of players' actions, the game aims to foster enhanced awareness of sustainability at both attitudinal and behavioral levels. 

This approach allows us to explore the following research questions:

\textbf{RQ1:} How can we design GenAI-driven conversational interactions to prompt players' in-game actions and enhance their sustainability awareness?

\textbf{RQ2:} What relationships exist between players' attitudes towards sustainable behavior and their in-game interactions?

Our research addresses those research questions through the following contributions:

\begin{itemize}
\item (a) Game Framework: 
Players navigate through various scenarios, understanding the long-term impact of their actions on the environment and society. By aligning in-game actions with real-life behaviors, we encourage players to reflect on their lifestyle and motivate them to translate these insights into real-world changes.

\item (b) Game Mechanism:
Our GenAI game strategy converts sustainability-related interactions between players and multimodal agents into in-game actions based on an intent-detection mechanism. The System dynamically adjusts their responses based on player choices and interactions, creating a realistic simulation of the consequences of these behaviors~\cite{8410872}. This design enables us to reliably capture player intent and assess the relationship between their attitudes and in-game behaviors, leading to more effective interventions for sustainable actions.


% \item (b) Intent Detection: 
% AI-driven NPCs dynamically adjust responses based on player choices and interactions, creating a more realistic simulation of behavioral consequences ~\cite{8410872}. This design enables us to accurately capture player intent and assess the relationship between their attitudes and in-game behaviors, leading to more effective interventions for sustainable actions.

\item (c) Empirical Study: 
We assessed changes in players' sustainability attitudes and behaviors before and after gameplay using surveys and semi-structured interviews. We found a significant increase in intended sustainable behaviors post-game, though attitudes only slightly improved.
% Notably, the design did not require altering players' personalities or mindsets, yet they still demonstrated a strong intention to engage in sustainable actions. This suggests that the game's influence on behavior can be effective across diverse audiences, regardless of their initial level of sustainability awareness.
% We analyzed changes in players' sustainability attitudes and behaviors before and after the game. Our data collection included pre- and post-game surveys and semi-structured interviews. The results showed a significant increase in intended sustainable behaviors after the game, while changes in sustainability attitudes were less pronounced, with only a slight improvement post-test. Interestingly, this game design does not require changing players' underlying personality or deeply-held beliefs. Even with relatively unchanged attitudes, participants still demonstrated a strong willingness to engage in sustainable actions. This suggests that the game's impact on behavior may be effective for different audiences, including those with varying levels of sustainability awareness. By allowing players to experience the long-term consequences of their actions in the game, we provide a flexible framework for promoting real-world sustainable behavior.
\end{itemize}


% CONTRIBUTION: we created a design where we do not even need to change people's personality / way of thinking, and not even change everybody, but by play the game they can still intend to take the sustainability course.
% (discussion: a republican climate denier can play this game and still turn off their aircon: 1. don't care their preexisting attitude, 2. don't care if you even changed their attitude -> intended change.)





% The proliferation of Generative AI has accustomed humans to prompting AI models to accomplish a diverse array of tasks. However, the capabilities of AI represent a double-edged sword; if utilized improperly, they may potentially lead to adverse consequences, such as unsustainable outcomes. This risk is particularly concerning as unsustainable behaviors are often imperceptible to individuals, given that the consequences of their actions are not immediately apparent. 

% The proliferation of Generative AI has accustomed humans to prompting AI models with encoded world knowledge to achieve various goals, such as code generation \cite{roziereCodeLlamaOpen2024} and image creation. However, can Generative AI utilize its encoded world knowledge to prompt humans and influence their goals?

% To explore this reversal of roles, it is required to ensure AI influences human goals in a positive way without negative or even malicious intent, and motivate humans to engage in meaningful dialogue with AI, allowing for potential "prompting" effects. To meet these criteria, we choose promoting human awareness of sustainable behaviors, a goal aligned with positive societal impact, as the task of our study. We employ a gamified framework to enhance user engagement and motivation for interaction with AI, creating an environment conducive to studying human-AI dynamic.
   

% \textbf{RQ1:} \textit{1} Can Generative AI accurately identify and interpret player inputs to match specific in-game task requirements?

% \textbf{RQ1:}  How do we design an AI-powered text-adventure game to promote sustainable awareness among players?

% \textbf{RQ2:} How do we use generative AI in supporting a sustainable awareness game development?
%something about using in-game measurements to see if they have sustainable attitude? correlates with survey perhaps.

% RQ1: How may we raise awareness for sustainable behavior by converting a natural-language-based verbal interaction into game actions?
% % %answer by creating the evaluation in-game.

% % %RQ: How can generative AI support the development of a game that promotes sustainable awareness?

% RQ2: How do we discover the attitudes of players towards sustainable behavior through their in-game interactions?
% % %1. in-game allocation, 2. verbal with chatgpt.
